Probabilistic Program Verification via Inductive Synthesis of Inductive Invariants

Essential tasks for the verification of probabilistic programs include bounding expected outcomes and proving termination in finite expected runtime. We contribute a simple yet effective inductive synthesis approach for proving such quantitative reachability properties by generating inductive invariants on source-code level. Our implementation shows promise: It finds invariants for (in)finite-state programs, can beat state-of-the-art probabilistic model checkers, and is competitive with modern tools dedicated to invariant synthesis and expected runtime reasoning.

==> conclusion.tex <==
\label{sec:conclusion}
We have developed an inductive invariant synthesis method for proving bounds on quantitative properties of probabilistic programs on source-code level.
Our prototype implementation shows promise: It can find invariants for a variety of verification problems and is competitive with state-of-the-art tools.
Future work includes incorporating nondeterminism and exploring advanced template shapes.
%
%This paper presents a novel inductive synthesis approach to probabilistic inductive invariants on probabilistic programs. We show the successful application to probabilistic program verification problems in general and probabilistic model checking in particular. Future work includes incorporating nondeterminism and accelerating the inductivity checks for large programs. Furthermore, we plan to explore advanced template shapes and heuristics to obtain diverse counterexamples.\mccomment{To be updated.}

==> pgcl.tex <==
% !TEX root = ./main.tex


The \emph{probabilistic Guarded Command Language} (\pgcl) adheres to the grammar%
%
\begin{align*}
	%
     \cc \quad{}\longrightarrow{}\quad %\qqlongrightarrow 
	%
	%
	 &\SKIP	\qmid \ASSIGN{x}{\ee}  \qmid  \COMPOSE{\cc}{\cc} %\tag{sequential composition}\\
	%
     \qmid  \PCHOICE{\cc}{p}{\cc} \qmid \\
    % \tag{probabilistic choice}\\
	%
      & \ITE{\guard}{\cc}{\cc} \qmid \WHILEDO{\guard}{\cc}~,
	%
\end{align*}%
%
where $\PCHOICE{\cc_1}{p}{\cc_2}$ is a probabilistic choice executing $\cc_1$ with probability \mbox{$p \in [0,1] \cap \Rats$} and $\cc_2$ with probability $1-p$. 
All other constructs have the usual meaning.\cmcomment{we should at least say what $\guard$ and $e$ are}
\emph{All while loops $\WHILEDO{\guard}{\mathtt{body}}$ in this paper have a loop free $\mathtt{body}$.}\footnote{Any \pgcl program with nested loops can be effectively transformed into a non-nested single-loop program~\cite{something} and our tool can perform such a transformation.}\cmcomment{move to problem statement?}
\cmcomment{I'm undecided: should we remove loops from the grammar or add their wp to the table? :)}

We assume an arbitrarily large, but \emph{finite}, set $\Vars$ of program variables~$x$.
Our program states in $\States = \setcomp{ \state}{\state\colon \Vars \to \Nats }$ map program variables to natural numbers.
A while loop $\WHILEDO{\guard}{\mathtt{body}}$ with loop-free $\mathtt{body}$ is \emph{finite-state}, if only finitely many states satisfy the loop guard $\varphi$, i.e.\  if $\bigl| \setcomp{\state \in \States }{ \state \models \guard} \bigr| < \infty$.

As linearity is pervasive in our approach, all expressions $e$ occurring in our programs shall be \emph{linear} (more precisely: \emph{affine}) in the program variables.
Also all guards $\guard$ are linear, i.e.\ they are arbitrary Boolean combinations of atoms of the form $\ee_1 < \ee_2$, where the $\ee_i$ are linear expressions.
For assignments, $\ASSIGN{x}{\ee}$, we need to (and in fact our tool \emph{can}) statically ensure that they are type-safe, i.e.\ the right-hand-sides need to always evaluate to $\Nats$ (in particular not into $\Ints_{{<} 0}$).

%\input{pgcl_grammar}

As promised earlier, we will now describe how to define the $\Phi$ function from \Cref{sec:overview} for any loop systematically. 
Let us first note that in \Cref{sec:overview} we considered whether final states met some target condition or not, which amounts to assigning a quantity in $\{0,\, 1\}$ to each final state.
We can, however, also assign quantities of type $\PosRealsInf$ outside the Boolean domain $\{0,\, 1\}$ to final states.
We call quantity assignments $f$ of type $\States \to \PosRealsInf$ \emph{expectations}.\footnote{\emph{Read:} expectation; \emph{think:} random variable.}
We denote the set of all expectations by $\E$, i.e.\ %
%
\begin{align*}
	\E \eeq \setcomp{f}{f \colon \States \to \PosRealsInf}~,\qquad \!\textnormal{where}\!\qquad f \ppreceq g \qiff \forall\, s \in \States\colon f(s) \leq g(s)~.
\end{align*}%
%
$\preceq$ is a partial order on $\E$ -- necessary to sensibly speak about least fixed points.

Recall that the sum appearing in the definition of $\Phi$ in \Cref{sec:overview}, namely%
%
\begin{align}
	\sum_{s' \in \States} \: \eval{\mathtt{body}}(s)(s') \cdot f(s')
	\label{eq:bodysum}
\end{align}%
%
is the expected value of $f$ (notice that $f \in \E$) evaluated in the final states reached after executing $\mathtt{body}$ on $s$.
By considering an arbitrary $\state$, \Cref{eq:bodysum} becomes an expectation of type $\E$, mapping initial states to expected values.
That is, we obtain precisely the so-called \emph{weakest preexpectation} of $C$ with respect to $f$~\cite{McIverM05,benni_diss}, denoted $\wp{\mathtt{body}}{f}$, \ie %
%
\begin{align*}
	\wp{\mathtt{body}}{f} \eeq \lambda\, \state.~\sum_{\state' \in \States} \: \eval{\mathtt{body}}(\state)(\state') \cdot f(\state')~.
\end{align*}
%
For any loop-free program $C$ and (post)expectation $f$, the weakest preexpectation $\wp{C}{f}$ can be defined purely syntactically and compositionally by induction on the structure of $C$, namely according to the rules in \Cref{table:wp}.%
%
%
\begin{table}[t]

	\renewcommand{\arraystretch}{1.5}

\begin{center}
\begin{tabular}{@{\hspace{1em}}l@{\hspace{2em}}l}
	\toprule
	$\boldsymbol{\cc}$			& $\boldsymbol{\textbf{\textsf{wp}}\,\left \llbracket \cc\right\rrbracket  \left(f \right)}$ \\
	\midrule
	$\SKIP$					& $f$ 																					\\
	%
	$\ASSIGN{x}{\ee}$			& $f\subst{x}{\ee}$ \\
	%
	$\COMPOSE{\cc_1}{\cc_2}$		& $\wp{\cc_1}{\vphantom{\big(}\wp{\cc_2}{f}}$ \\
	%
	$\PCHOICE{\cc_1}{\pp}{\cc_2}$		& $\pp \cdot \wp{\cc_1}{f} + (1- \pp) \cdot \wp{\cc_2}{f}$ \\
	%
	$\ITE{\guard}{\cc_1}{\cc_2}$		& $\iverson{\guard} \cdot \wp{\cc_1}{f} + \iverson{\neg \guard} \cdot \wp{\cc_2}{f}$ \\[.25em]
	%
%    $\WHILEDO{\guard}{\cc'}$		& $\lfp X\mydot \iverson{\neg \guard} \cdot f + \iverson{\guard} \cdot \wp{\cc'}{X}$ \\
	\bottomrule
\end{tabular}
\end{center}
\caption{Rules defining the weakest preexpectation transformer for loop-free programs. 
$\iverson{\varphi}$ denotes an indicator function, \ie $\iverson{\varphi}(s) = 1$ if $s \models \varphi$ and $0$ otherwise.}
\label{table:wp}
\end{table}
%
%

For a general loop $\WHILEDO{\guard}{C}$ we now want to characterize the expected value of $f$ after termination of the loop on initial state $\state$.
For \emph{any} initial state, this can be characterized as the least fixed point of the function%
%
\begin{align*}
	\charfun{f}(X) \eeq \iverson{\neg \guard} \cdot f \pplus \iverson{\guard}\cdot \wp{C}{X}~.
\end{align*}
%
Intuitively, to any state $s$ that does not satisfy the loop guard $\guard$, we assign directly the terminal quantity $f(s)$.
To all other states that \emph{do} satisfy the loop guard, we assign the expected value of $X$ after one more loop body iteration.
Indeed, the least fixed point of $\charfun{f}$ is precisely the weakest preexpectation of the entire loop with respect to $f$, \ie %
%
\begin{align*}
	\wp{\WHILEDO{\guard}{C}}{f} \eeq \lfp \charfun{f}~.
\end{align*}%
%
In words: $\lfp \charfun{f}$ maps any initial state $s$ to the expected value of $f$ evaluated in the final states that are reached after termination of $\WHILEDO{\guard}{C}$ on $s$.


==> pgcl_grammar.tex <==
% !TEX root = ./main.tex

\begin{figure}[t]
\begin{adjustbox}{max width=\textwidth}
\begin{minipage}[t]{0.33\linewidth}
\begin{align*}
	%
     \cc ~\longrightarrow~ %\qqlongrightarrow 
	%
	%
	& \SKIP	\\%\tag{effectless program} \\
	%
    \qmid & \ASSIGN{x}{\ee} \\%  \tag{assignment}\\
	%
    \qmid & \COMPOSE{\cc}{\cc} \\%\tag{sequential composition}\\
	%
    \qmid & \PCHOICE{\cc}{p}{\cc}  \\
    % \tag{probabilistic choice}\\
	%
    \qmid & \ITE{\guard}{\cc}{\cc} \\%\tag{conditional choice} \\
    %
    \qmid & \WHILEDO{\guard}{\cc'}
	%
\end{align*}
\subcaption{$\pgcl$ programs}
\label{fig:grammars:pgcl}
\end{minipage}
\begin{minipage}[t]{0.43\linewidth}
\begin{align*}
\ee ~\longrightarrow~
   %
   & z \\ %\tag{constants} \\
   %
   \qmid & x \\ %\tag{$\Nats$-valued variables}\\
   %
   %
   \qmid & z \cdot \ee  \\ %\tag{multiplication by $\mathbb{A}$-valued constants}\\
   %
   %
   \qmid & \ee+\ee  \\ %\tag{addition}\\
   %
   %
   \\
\end{align*}
\subcaption{Linear expressions over $\Vars$ with coefficients in $\Ints$.}
\label{fig:grammars:expressions}
\end{minipage}
\begin{minipage}[t]{0.2\linewidth}
\begin{align*}
\guard ~\longrightarrow~
   %
   %
   & \ee < \ee  \\ %\tag{strict inequality of arithmetic expressions in $\aexplinpar{\mathbb{A}}$} \\
   %
   %
   \qmid & \guard \wedge \guard \\% \tag{conjunction} \\
   %
   %
   \qmid & \neg \guard %\tag{negation}
    \\
    \\
    \\
\end{align*}
\subcaption{Linear guards}
\label{fig:grammars:guards}
\end{minipage}
\end{adjustbox}
\caption{
  Syntax of $\pgcl$ programs, linear expressions, and guards,
  where $x \in \Vars$ (evaluating to natural numbers),
  $p \in [0,1] \cap \Rats$ is a rational probability, 
  and $z \in \Ints$ is a constant.
}
\label{fig:grammars}
\end{figure}


==> problem.tex <==
% !TEX root = main.tex





%\subsection{Expectations and Templates}
\cmcomment{Expectations were defined in the prev. section; syntactic or linear expectations?}

\subsubsection{Linear Expectations}
To allow for efficiently checking whether a candidate invariant is indeed inductive, we restrict ourselves to \emph{piecewise} linear expressions\cmcomment{I first read expectation given the section title :)}:
\begin{definition}
	The set $\aexp$ of \emph{linear expressions over $\Vars$ with coefficients in $\Rats$} is given by the grammar
	%
	\begin{align*}
		\ea \quad\longrightarrow \quad
		\rr + \sum\limits_{i=1}^{n} \rr_i \cdot x_i,~\text{where $\rr,\rr_i \in \Rats$}~.
	\end{align*}
 %
 %
 %
 The set $\bexp$ of \emph{Boolean expressions over $\aexp$} is given by the grammar
 %
 \begin{align*}
 	\bb \quad\longrightarrow \quad
 	%
 	~ \ea <\ea ~\mid~\bb \wedge \bb ~\mid~ \neg \bb~.
 	\tag*{$\triangle$}
 \end{align*}

\end{definition}

\begin{definition}
	\emph{Piecewise linear expectations} $f \in \Elin$ and $g \in \Elininf$ adhere to the grammar
	%
	\[
	   f \quad \longrightarrow  \quad \sum\limits_{i=1}^{N}   \iverson{\bb_i} \cdot \ea_i
	   \qquad \text{and} \qquad
	   g \quad \longrightarrow  \quad \sum\limits_{i=1}^{N}   \iverson{\bb_i} \cdot \eainfty_i
	\]
	%
	where $\eainfty_i \in \aexp \cup \{\infty\}$, $N \geq1$, and 
	\begin{enumerate}
		%
		\item for all $i \in \{1,\ldots,N\}$ and all $\sigma \in \States$, $\sigma \models \bb_i$ implies $\ea_i(\sigma) \geq 0$ (resp.\ $\eainfty_i(\sigma) \geq 0$), and
		%
		%
		\item the Boolean expressions $\bb_1,\ldots,\bb_N$ partition the state space $\States$, i.e., for every $\sigma \in \States$ there is \emph{exactly one} $\bb_i$ with $\sigma \models \bb_i$. \hfill $\triangle$
	\end{enumerate}
\end{definition}

%As we outlined above, we aim to solve the problem of finding an inductive invariant (of a particular shape) by solving three problems:
%
%
%Towards solving this problem, we assume that for any $\inv \in \Elin$ there exists an efficient verifier that solves the verifier problem:
%\begin{mdframed}
%	 \textbf{Verifier problem}: Given $\inv \in \Elin$, decide if $\inv \in \indinvshort$.
%\end{mdframed}
%%
%
%
\subsubsection{Expectation Templates}
%
Instead of searching through all piecewise linear expectations, we restrict ourselves to a set which is described by \emph{templates}.

Let $\tvars$ be a countably infinite set of $\Rats$-valued \emph{template variables}, denoted by $\alpha, \beta,\ldots$. We call $\tval \colon \tvars \to \Rats$ a \emph{(template variable) valuation}.


\begin{definition}
	The set $\taexp$ of \emph{templated linear expressions over $\Vars$ with coefficients in $\Rats \cup \tvars$} is given by the grammar
	%
	\begin{align*}
		\et \quad\longrightarrow \quad
		\rt + \sum\limits_{i=1}^{n} \rt_i \cdot x_i,~\text{where $\rt,\rt_i \in \Rats \cup \tvars$}~.
	\end{align*}
   %
	%
	%
	%
	The set $\tbexp$ of \emph{templated Boolean expressions over $\taexp$} is given by the grammar
	%
	\begin{align*}
		\bt \quad\longrightarrow \quad
		%
		~ \et <\et ~\mid~\bt \wedge \bt ~\mid~ \neg \bt~.
		\tag*{$\triangle$}
	\end{align*}
	%
\end{definition}
%
Given a valuation $\tval$ and $\et \in \taexp$ (resp.\ $\bt \in \tbexp$), the linear expression (resp.\ Boolean expression) obtained from substituting every occurrence of a template variable $\alpha$ in $\rt$ (resp.\ in $\bt$) is denoted by $\tvalapps{\et}\in \aexp$ (resp. $\tvalapps{\bt} \in \bexp$). 
%

An \emph{expectation template} $\temp$ is an expression generating a (possibly infinite) set of linear expectations.
%
%
\begin{definition}
	\emph{Linear expectation templates} (\emph{templates}, for short) $\temp \in \TElin$ adhere to the grammar
	%
	\begin{align*}
	\temp \quad \longrightarrow  \quad \sum\limits_{i=1}^{N}   \iverson{\bt_i} \cdot \et_i~, \text{where $N\geq1$}
	\end{align*}
	%
	such that for every valuation $\tval$ the Boolean expressions $\tvalapps{\bt_1},\ldots,\tvalapps{\bt_N}$ partition the state space $\Sigma$. \hfill $\triangle$
\end{definition}
%
We denote the expression obtained from substituting every occurrence of a template variable $\alpha$ in $\temp$ by $\tvalapps{\temp}$. We might have $\tvalapps{\temp} \not\in \Elin$. We define
%
\[
   \generator{\temp} \eeq \left\{ \tvalapps{\temp} ~\mid~ \tval \colon \tvars \to \Rats \right\}~.
\]
%
In this paper, we consider two types of templates:
%
\begin{definition}
	A \emph{fixed-partition template} is a template $\temp \in \TElin$ of the form
	%
	\begin{align*}
	\temp \eeq \sum\limits_{i=1}^N  \iverson{\bb_i} \cdot \et_i~
	\tag*{$\triangle$}
	\end{align*}
	%
\end{definition}
%
%
\begin{definition}
\label{def:vptemplates}
	A \emph{variable-partition template} is a template $\temp \in \TElin$ of the form
	\begin{align*}
	\temp \eeq \sum\limits_{i=1}^N  \iverson{\bb_i \wedge \bt_i} \cdot \et_i
	\tag*{$\triangle$}
	\end{align*}
	%
	where each $\bt_i$ is a conjunction of inequalities of the form $x\leq\lambda$ or $\lambda <x$ for $x \in \Vars$ and $\lambda \in \tvars$. %and where the Boolean expressions $\bb_i \wedge \tvalapps{\bt_i}$ partition the state space $\States$ for all $\tval$. \hfill $\triangle$
\end{definition}


\subsubsection{Formal Problem Statement}
We are now ready to to formalise the problem statement.
%
In the sequel, fix a single-loop $\cc = \WHILEDO{\guard}{\cc'}$ and $f,g \in \Elin$ with $\wp{\cc}{f} \leq g$. Denote by $\charfun{g}$ the characteristic functional of $\cc$ w.r.t.\ postexpectation $g$.\cmcomment{Choose something more descriptive like loop, guard, body, pre post?} Let 
%
\[
    \indinv  \eeq \left\{ \inv \in \Elin ~\mid~ \charfun{f}(\inv) \leq \inv ~\text~{and}~ \inv \leq g \right\}~.
\]
%
For conciseness, we denote $\indinv$ as $\indinvshort$.

\begin{mdframed}
	 \textbf{Formal problem statement}: Given template $\temp$, find $\inv \in \generator{\temp}$ with $\inv \in \indinvshort$ or determine that there is no such $\inv \in \generator{\temp}$.
\end{mdframed}
%
Templates can be either fixed-partition templates or variable-partition templates. 
Notice that we might have $\indinvshort = \emptyset$  since in general more complex expectations are needed (cite relative completeness). However,
%
\begin{theorem}
	If $\cc$ is finite-state, then $\indinvshort \neq \emptyset$.
\end{theorem} 
\begin{proof}
Let $I = \wp{\cc}{f} = \lfp \charfun{f}$.\cmcomment{Note that $I$ maps every state to a rational and give a citation}
Clearly, $\Phi_f(I) = \Phi_f(\lfp \charfun{f}) = \lfp \Phi_f = I \leq I$ and, by definition, $I \leq g$.

It remains to show that we can write $I$ as a linear expectation whenever $\cc$ is finite-state.
To this end, let $S' = \{ \state \mid \state \models \guard \}$ denote the finite set of states satisfying the loop guard, and recall that the set $\Vars$ of variables is finite. Then:\cmcomment{technically, one needs to write $\neg x < \state(x) \wedge \neg \state(x) < x$ given the current syntax?}
\begin{align*}
	I \eeq & \charfun{f}(I) \eeq \iverson{\neg \guard} \cdot f + \iverson{\guard} \cdot \wp{\cc'}{I} \\
	  \eeq & \iverson{\neg \guard} \cdot f + \iverson{\guard} \cdot \sum_{\state \in \States} \iverson{\bigwedge_{x \in \Vars} x = \state(x)} \cdot \wp{\cc'}{I}(\state) \\
	   \eeq & \iverson{\neg \guard} \cdot f + \sum_{\state \in \States'} \iverson{\guard \wedge \bigwedge_{x \in \Vars} x = \state(x)} \cdot \underbrace{\wp{\cc'}{I}(\state)}_{\text{TODO: this is rational, because...?}} \\
	   ~\in~ & \Elin~. \tag*{\qed}
\end{align*}
\end{proof}

\cmcommentinline{Put the templates we consider here.}


\section{One-Shot Synthesis}
One approach towards our formal problem statement is to \emph{ignore} the presence of a verifier and solve the problem in a single shot rather than iteratively. While this approach does not scale, it inspires the iterative approach.
\kbcommentinline{examples.. use running example from overview section to illustrate things}
\begin{lemma}
	\label{lem:inv_is_indinv}
	Let $\temp$ be a template and $\inv \in \generator{\temp}$. We have  $\inv \in \indinvshort$ iff
	%
	\begin{enumerate}
		\item \emph{well-definedness}:  $\inv \geq 0$,
	%\end{enumerate}
	%
	%If $\inv \in \Elin$ we moreover have $\inv \in \indinvshort$ iff
	%
	%\begin{enumerate}
		\item[2.] \emph{inducitivity}: $\charfun{f}(\inv)\leq \inv$, and
		%
		\item[3.] \emph{safety}: $ \inv\leq g$.
	\end{enumerate}
\end{lemma}
\cmcommentinline{The above lemma seems a bit superfluous?}
\begin{theorem}
	\label{thm:templatetrans}
	Let $\cc = \WHILEDO{\guard}{\cc'}$ be a single-loop and let $f \in \Elin$. There is an computable map 
	%
	\[
	\tcharfun{f} \colon \TElin \to \TElin 
	\quad
	\text{such that}
	\quad
	\forall \temp \colon \forall \tval \colon
	\tvalapps{\tcharfun{f}(\temp)} = \charfun{f}(\tvalapps{\temp})~.
	\]
	\cmcomment{Strictly speaking, $\charfun{f}(\tvalapps{\temp})$ is not well-defined?}
	%
\end{theorem}
%
\begin{proof}
  For loop-free $\pgcl$ programs, we lift the transformer
  $\wpsymbol$ in \Cref{table:wp} to a transformer
  in which expectations can have template parameters; the rules are exactly the same as in \Cref{table:wp}---only the underlying types change.
  Furthermore, we define $\tcharfun{f}$ on expectations with template parameters analogously to the characteristic function $\charfun{f}$, \ie 
  \[
      \tcharfun{f}(\temp) \eeq \iverson{\neg \guard} \cdot f \pplus \iverson{\guard}\cdot \wp{\cc'}{\temp}~.
  \] 
  Now, let $\temp \in \TElin$ and $\tval$ be a template
  valuation. Then:
  \begin{align*}
    	\tvalapps{\tcharfun{f}(X)} \eeq & 
    	\tvalapps{\left(\iverson{\neg \guard} \cdot f \pplus \iverson{\guard}\cdot \wp{\cc'}{\temp}\right)} \\
    	\eeq & \tvalapps{(\iverson{\neg \guard} \cdot f)} \pplus \tvalapps{(\iverson{\guard}\cdot \wp{\cc'}{\temp})} \\
    	\eeq & \iverson{\neg \guard} \cdot f \pplus \iverson{\guard}\cdot \tvalapps{\wp{\cc'}{\temp}} \tag{$\guard$, $f$ contain no parameters} \\
    	\eeq & \iverson{\neg \guard} \cdot f \pplus \iverson{\guard}\cdot \wp{\cc'}{\tvalapps{\temp}} \tag{by induction, see below} \\
    	\eeq & \charfun{f}(\tvalapps{\temp})~.
  \end{align*}
  The missing step from above follows from a straightforward by structural induction on $\cc'$ (\ie, loop-free $\pgcl$ programs), that is, 
  \[
     \forall \temp \colon \: \forall \tval \colon \qquad
	\tvalapps{\wp{\cc'}{\temp}} \eeq \wp{\cc'}{\tvalapps{\temp}}~.
  \]
  To complete the proof, notice that $\tcharfun{f}$
  can be written as a linear expectation template (\ie $\tcharfun{f} \in \TElin$) using the construction in \cite[Lemma 3 and Section 7.1]{DBLP:conf/cav/BatzCKKMS20}, where all template parameters are treated as constants.\cmcomment{put details in appendix; split theorem into two?}
  \qed
\end{proof}
%
\kbcomment{say that size of $|\tcharfun{f}(\temp)| =|\charfun{f}(\inv)|$ (if it is actually true) and mention the exponential blow-up. Does it matter in practice?}
%
%
For simplicity, we restrict to fixed-partition templates $\temp$. Given $\et \in \taexp$ and $\sigma \in \States$, we denote by $E(\sigma)$ the linear expression over $\tvars$ with coefficients in $\Rats$ obtained from substituting every program variable $x$ in $E$ by $\sigma(x)$. Moreover, given $\temp \in \TElin$ as above, we define
%
\[
T(\sigma) \eeq \et_j(\sigma)\quad\text{for $j$ with $\sigma \models \bb_j$}~.
\]
%
Recall that there is exactly one $j$ such that $\sigma \models \bb_j$. 
In the following, given an FO-formula $\phi$ (with a fixed underlying structure) and suitable variable valuation $\tval$, we write $\tval \models \phi$ to indicate that $\tval$ satisfies $\phi$. Moreover, we define 
%
\[
    \satset(\phi) \eeq  \left\{ \tval ~\mid~ \tval \models \phi \right\}~.
\]


\begin{theorem}
	For fixed-partition template $\temp \in \TElin$, we have
	%
	\begin{align*}
	&\exists \inv \in \generator{\temp}\colon \inv \in \indinv \\
	%
	\text{iff} \quad &
	%
	 \satset\left(\forall\sigma \in \States \colon 
	0 \leq \temp(\sigma) \wedge \tcharfun{f}(\temp)(\sigma) \leq \temp(\sigma) \wedge \temp(\sigma) \leq g(\sigma)\right)\neq \emptyset %\\
	%& \text{is satisfiable}~.  
	\end{align*}
\end{theorem}
%


\begin{proof}
%
%
We have
	\begin{align*}
	&\exists \inv \in \generator{\temp}\colon \inv \in \indinv \\
    %
    \text{iff} \quad &\exists \inv \in \generator{\temp}\colon
    	0 \leq \inv \wedge \charfun{f}(\inv) \leq \inv \wedge \inv \leq g  
    	\tag{by \Cref{lem:inv_is_indinv}}\\
    %
     \text{iff} \quad &\exists \inv \in \generator{\temp}	\colon \forall\sigma \in \States \colon 
    0 \leq \inv(\sigma) \wedge \charfun{f}(\inv)(\sigma) \leq \inv(\sigma) \wedge \inv(\sigma) \leq g(\sigma) 
    \\
    %
    \text{iff} \quad &\exists \tval 	\colon \forall \sigma \colon 
    0 \leq \tvalapps{\temp}(\sigma) \wedge \charfun{f}(\tvalapps{\temp})(\sigma) \leq \tvalapps{\temp}(\sigma) \wedge \tvalapps{\temp}(\sigma) \leq g(\sigma)  \\
    %
    \text{iff} \quad &\exists \tval 	\colon \forall\sigma  \colon 
    0 \leq \tvalapps{\temp}(\sigma) \wedge \tvalapps{\tcharfun{f}(\temp)}(\sigma) \leq \tvalapps{\temp}(\sigma) \wedge\tvalapps{\temp}(\sigma) \leq g(\sigma)  
    \tag{by \Cref{thm:templatetrans}}\\
    %
    \text{iff} \quad &\satset\left(\forall\sigma\colon 
    0 \leq \temp(\sigma) \wedge \tcharfun{f}(\temp)(\sigma) \leq \temp(\sigma) \wedge \temp(\sigma) \leq g(\sigma)\right)\neq \emptyset 
    \end{align*}
\kbcomment{Use different symbol for constraint $\leq$}
\end{proof}
%
%
%
\kbcommentinline{keep in mind that $T$ must be of this shape! also for completeness of algo. or assume that $T$ is always of this shape.}
\begin{theorem}
	Let $\temp$ be a fixed-partition template of the form
	\[
	    \temp \eeq \iverson{\neg \guard}\cdot f + \sum\limits_{i=1}^N  \iverson{\bb_i} \cdot \et_i~
	\]
	%
	and assume $\iverson{\neg \guard}\cdot f \leq \iverson{\neg \guard} \cdot g$\kbcomment{this must not be assumed. It follows from $\wp{\cc}{f}\leq g$}. If $\cc$ is finite-state, then $\exists \inv \in \generator{\temp}\colon \inv \in \indinv$ is decidable by solving a system of finitely many linear inequalities.
\end{theorem}
%
\begin{proof}
	TODO.
\end{proof}
%
Notice that the above $\bb_i$ necessarily partition $\guard$.

%



==> rebuttal.tex <==
We are grateful for the reviewer's valuable and constructive feedback. All suggestions will be taken into account for the final version of the paper. Below we address the main criticism raised by Reviewer 2.


"The probabilistic feature of the language doesn't really play a role [...]"

Even though the semantic treatment might seem straightforward, introducing randomization by adding a probabilistic choice statement causes challenging phenomena: We encounter dense search spaces even for finite-state programs (since inductive invariants are of type States -> NonNegativeReals) and the related fact that one generally needs richer arithmetic theories such as mixed linear integer- and real arithmetic. Moreover, many techniques from the non-probabilistic setting rely on the fact that a counterexample to safety is a *single path* ending in an unsafe state. In the probabilistic setting, however, counterexamples generally consist of *sets* of possibly cyclic paths whose accumulated probability mass exceeds a certain threshold. This has been recognized as a severe issue when, e.g., generalizing CEGAR [A] or IC3 [11] to the probabilistic setting and is particularly challenging when verifying lower bounds on reachability probabilities. It was, therefore, a-priori unclear whether adopting a CEGIS approach to the probabilistic setting is feasible.



"[...] the "quality" of the invariants cannot be easily assessed."

We agree that it is not easy to assess how far away a given inductive invariant I is from the "actual" reachability probabilities. All we know is that I was good enough to certify the validity of the given property. This is analogous to classical Hoare-style reasoning and the majority of state-of-the-art symbolic verification techniques for both non-probabilistic and probabilistic programs, e.g. IC3/PDR [B] or interpolation [C] - and template-based [1,9,24,28,31,54] techniques. For instance, suppose we aim to verify a Hoare triple {P} C {Q} of a loop C using a loop invariant I. There might be weaker (i.e., "tighter") invariants I'. However, I was good enough to certify the validity of the given Hoare triple. We remark that our comparison to the Absynth tool [49] provides some indication of the quality of our invariants when comparing to alternative approaches: Even though Absynth is optimized towards finding tight runtime bounds, our approach often finds bounds of similar quality (cf. Appendix E.2).


"The settings are simple: no nested loops [...]"
Considering only non-nested loops is not a restriction since every nested loop can be automatically transformed into a non-nested loop.

"The generated invariants serve only the purpose of proving the property, they don't characterize the program in anyway."

An inductive invariant typically contains more information than the property that is to be verified. Consider, for instance, the inductive invariant I for the bounded retransmission protocol depicted in Figure 3b. Since I overapproxiamtes the probability to reach an error state for *all* states, we can read off those overapproximations not only for the initial state of the program but also for intermediate states. 


Regarding the fact that limiting the synthesizer to a small number of states is able to generate global invariants.
"Is it specific to certain kind of benchmarks? Or is it more related to the properties one would like to prove?"

Both the program and the property can have a significant impact on the number of required CTIs. For instance, we observe from Table 2 in Appendix E.1 that there are programs (gridsmall) with a small state space that require a relatively high amount of CTIs. On the other hand, for a fixed program (e.g. zeroconf), the number of required CTIs can vary drastically depending on the tightness of the considered threshold on the reachability probabilities.

We agree that a deeper theoretical investigation is a great direction for future work. 


===References===

[A] Hermanns et al.: Probabilistic CEGAR. CAV’08.
[B] Bradley. SAT-Based Model Checking without Unrolling.
[C] McMillan. Lazy Abstraction with Interpolants.






==> table_infinite_state.tex <==
%\begin{table}[t]
%\begin{subtable}[t]
\caption{CEGIS on inf.-state programs, {\small{TO=2h}}. %Runtimes in seconds.
}\label{tab:infinite}
	\adjustbox{width=1\textwidth}{
\begin{tabular}{l||rrrr|rrrr|rrrr}
%\begin{tabular}{lrrrrrrrrrrrr}
	\toprule
	&     \multicolumn{8}{c}{\headername{inductivity-guided}} & \multicolumn{4}{c}{\headername{dynamic}}  \\ 
	&     \multicolumn{4}{c}{\headername{\prepsynthesizer}} & \multicolumn{4}{c}{\headername{plain}} \\ 
	\headername{Prog} & {\footnotesize $|S'|$}  & {\footnotesize $|T|$} &  {\footnotesize $\headername{t}_\text{s}$\%} & {\footnotesize \headername{t}} & {\footnotesize $|S'|$} & {\footnotesize $|T|$} & {\footnotesize $\headername{t}_\text{s}$\%}  & {\footnotesize \headername{t}} & {\footnotesize $|S'|$} & {\footnotesize $|T|$} & {\footnotesize $\headername{t}_\text{s}$\%}  & {\footnotesize \headername{t}} \\ 
	\midrule\midrule\multirow{3}{*}{\footnotesize{\expname{brpfam}}}&{\scriptsize $93$}&{\scriptsize $7$}&{\scriptsize $85$}&{\scriptsize $176$}&{\scriptsize $71$}&{\scriptsize $8$}&{\scriptsize $84$}&{\scriptsize $56$}&--&--&--&{\scriptsize TO}\\ 
	&{\scriptsize $47$}&{\scriptsize $7$}&{\scriptsize $79$}&{\scriptsize $39$}&{\scriptsize $76$}&{\scriptsize $8$}&{\scriptsize $88$}&{\scriptsize $102$}&--&--&--&{\scriptsize TO}\\ 
	&--&--&--&{\scriptsize TO}&--&--&--&{\scriptsize TO}&--&--&--&{\scriptsize TO}\\ 
	% 
	% 
	\midrule  
	\multirow{1}{*}{\footnotesize{\expname{eqgridfam}}}&{\scriptsize $6$}&{\scriptsize $4$}&{\scriptsize $62$}&{\scriptsize $1$}&{\scriptsize $14$}&{\scriptsize $4$}&{\scriptsize $51$}&{\scriptsize $1$}&{\scriptsize $14$}&{\scriptsize $4$}&{\scriptsize $95$}&{\scriptsize $9$}\\ 
	% 
	\midrule  
	\multirow{2}{*}{\footnotesize{\expname{geo}}}&{\scriptsize $1$}&{\scriptsize $2$}&{\scriptsize $25$}&{\scriptsize ${<}1$}&{\scriptsize $2$}&{\scriptsize $2$}&{\scriptsize $11$}&{\scriptsize ${<}1$}&{\scriptsize $2$}&{\scriptsize $2$}&{\scriptsize $10$}&{\scriptsize ${<}1$}\\ 
	&{\scriptsize $1$}&{\scriptsize $2$}&{\scriptsize $14$}&{\scriptsize ${<}1$}&{\scriptsize $2$}&{\scriptsize $2$}&{\scriptsize $12$}&{\scriptsize ${<}1$}&{\scriptsize $2$}&{\scriptsize $2$}&{\scriptsize $12$}&{\scriptsize ${<}1$}\\ 
	% 
	\midrule  
	\multirow{1}{*}{\footnotesize{\expname{kgeo}}}&{\scriptsize $2$}&{\scriptsize $2$}&{\scriptsize $20$}&{\scriptsize ${<}1$}&{\scriptsize $474$}&{\scriptsize $2$}&{\scriptsize $81$}&{\scriptsize $31$}&--&--&--&{\scriptsize TO}\\ 
	% 
	\bottomrule  
\end{tabular}
}
%\end{table}
%\end{table}
%\sjcomment{Use same fontsize (approx) for both tables}

==> table_oneshot.tex <==
%\begin{table}[t]
\caption{CEGIS vs.\ \mono, {\small{TO=30m}}. %Runtimes in seconds.
}\label{tab:innercegis}
\adjustbox{width=1\textwidth}{
\begin{tabular}{lc||r||rrr|rrr}
%\begin{tabular}{lcrrrrrrr}
	\toprule
	&   & \multicolumn{1}{c}{\mono} & \multicolumn{3}{c}{\headername{\prepsynthesizer}} & \multicolumn{3}{c}{\headername{plain}} \\ 
	\headername{Prog} & {\footnotesize $|T|$} & \headername{t} &  {\footnotesize $|S'|$}  &   {\footnotesize $\headername{t}_\text{s}$\%} & {\footnotesize \headername{t}} & {\footnotesize $|S'|$} & {\footnotesize $\headername{t}_\text{s}$\%} & {\footnotesize \headername{t}} \\ 
	\midrule\midrule\multirow{2}{*}{\footnotesize{\expname{rw}}}& 12 & {\scriptsize $33$}&{\scriptsize $33$}&{\scriptsize $28$}&{\scriptsize $15$}&{\scriptsize $32$}&{\scriptsize $20$}&{\scriptsize $9$}\\ 
	& 20 & TO&{\scriptsize $54$}&{\scriptsize $34$}&{\scriptsize $72$}&{\scriptsize $62$}&{\scriptsize $16$}&{\scriptsize $41$}\\ 
	% 
	% 
	\midrule  
	\multirow{2}{*}{\footnotesize{\expname{chain}}}& 5 & {\scriptsize $1$}&{\scriptsize $63$}&{\scriptsize $53$}&{\scriptsize $3$}&{\scriptsize $22$}&{\scriptsize $33$}&{\scriptsize $1$}\\ 
	& 23 & {\scriptsize $294$}&--&--&{\scriptsize TO}&--&--&{\scriptsize TO}\\ 
	% 
	\midrule  
	\multirow{2}{*}{\footnotesize{\expname{multchain}}}& 15 & TO&{\scriptsize $203$}&{\scriptsize $82$}&{\scriptsize $263$}&{\scriptsize $154$}&{\scriptsize $61$}&{\scriptsize $54$}\\ 
	& 15 & TO&{\scriptsize $186$}&{\scriptsize $80$}&{\scriptsize $205$}&{\scriptsize $141$}&{\scriptsize $59$}&{\scriptsize $51$}\\ 
	% 
	\midrule  
	\multirow{1}{*}{\footnotesize{\expname{gridsmall}}}& 17 & TO&{\scriptsize $69$}&{\scriptsize $36$}&{\scriptsize $16$}&{\scriptsize $77$}&{\scriptsize $25$}&{\scriptsize $12$}\\ 
	% 
	\midrule  
	\multirow{1}{*}{\footnotesize{\expname{0conf}}}	& 23 & {\scriptsize $111$}&{\scriptsize $175$}&{\scriptsize $64$}&{\scriptsize $1123$}&{\scriptsize $236$}&{\scriptsize $64$}&{\scriptsize $863$}\\ 
	% 
	\midrule  
	\multirow{1}{*}{\footnotesize{\expname{brpfam}}}& 7 & no inst.&{\scriptsize $63$}&{\scriptsize $84$}&{\scriptsize $70$}&{\scriptsize $63$}&{\scriptsize $96$}&{\scriptsize $356$}\\ 
	% 
	\midrule  
	\multirow{1}{*}{\footnotesize{\expname{0conffam}}}& 3 & {\scriptsize $2$}&{\scriptsize $34$}&{\scriptsize $52$}&{\scriptsize $2$}&{\scriptsize $37$}&{\scriptsize $42$}&{\scriptsize $2$}\\ 
	% 
	\bottomrule  
\end{tabular}


}		
%\end{table}

==> vptemplatesynt.tex <==
% !TEX root = ./main.tex


\label{sec:vptemplates}
We generalize the ideas from above to support variable-partition templates $\temp$ as formalized in Def.~\ref{def:vptemplates}. This generalization does not require any changes in the verifier since instances $\inv \in \generator{\temp}$ are still piecewise linear expectations.
However, to ensure that our implementation of $\tsynt$ is indeed a synthesizer, the constraints from \eqref{eq:syntimpl} on p.~\pageref{eq:syntimpl} must be modified. Let us motivate this generalization by an example.
\begin{example}
	Reconsider the variable-partition template $\temp$ in \Cref{eq:varpartemplexample}: \sjcomment{Possibiilty to save space by not restating this}
		 \begin{align*} 
		T \eeq 
		%
		& \iverson{\varfailed < 10 \land \varsent < \delta} \cdot \left( \alpha_1 \cdot \varsent + \beta_1 \cdot \varfailed + \gamma_1  \right) \pplus  \\
		%
		& \iverson{\varfailed < 10 \land \varsent \geq \delta} \cdot \left( \alpha_2 \cdot \varsent + \beta_2 \cdot \varfailed + \gamma_2 \right) \pplus \iverson{\varfailed=10} \end{align*}
	  %
	  %
	  and assume a counterexample $\state$ with $\state(\varfailed) = 5$ and $\state(\varsent) = 2$. Our goal is to construct an LRA formula over $\tvars$ ensuring that instances $\inv$ of $\temp$ are valid w.r.t.\ $\state$.
	  %Our goal is to ensure that future instances of $\temp$ will be valid w.r.t.\ $\state$. 
	  Since the partitioning of the state space is not fixed in $\temp$ but depends on the valuation of $\delta$, we need constraints for the cases where $\state$ belongs to $\iverson{\varfailed < 10 \land \varsent < \delta}$ \emph{and} where $\state$ belongs to $\iverson{\varfailed < 10 \land \varsent \geq \delta}$. The resulting constraints are conjunctions of implications. For instance, the constraints ensuring that an instance $\inv$ satisfies $\inv(s) \geq 0$ are
	  %
	  \[
	             (5<10 \wedge 2 < \delta) \Rightarrow \alpha_1 \cdot 2 + \beta_1 \cdot 5 + \gamma_1 \geq 0
	             ~\text{and}~
	              (5<10 \wedge 2 \geq \delta) \Rightarrow \alpha_2 \cdot 2 + \beta_2 \cdot 5 + \gamma_2 \geq 0
	  \]
	
\end{example}
%Thus, the encoding now is a conjunction of implications and therefore no longer a linear program. 
Thus, the conjunction of linear inequalities~\eqref{eq:syntimpl} becomes a conjunction over implications of linear inequalities\sjcomment{Do ew want to put these in the appendix or is it fine as is} and thus has a Boolean structure. 
Finally, we remark that for variable-partition templates it is \emph{not possible in general} to employ Motzkin's transposition theorem to obtain \emph{linear} constraints ensuring that instances $\inv \in \generator{\temp}$ satisfy $I(\state) \geq 0$ and $I(\state) \leq g(\state)$ for \emph{every} $\state$.

 %the Motzkin-based preprocessing of Sec.~\ref{} now would violate the linearity assumption:
%\begin{example}
	
%\end{example}

